Seeking Specifications: The Case for Neuro-Symbolic Specification Synthesis

This work is concerned with the generation of formal specifications from code, using Large Language Models (LLMs) in combination with symbolic methods. Concretely, in our study, the programming language is C, the specification language is ACSL, and the LLM is Deepseek-R1. In this context, we address two research directions, namely the specification of intent vs. implementation on the one hand, and the combination of symbolic analyses with LLMs on the other hand. For the first, we investigate how the absence or presence of bugs in the code impacts the generated specifications, as well as whether and how a user can direct the LLM to specify intent or implementation, respectively. For the second, we investigate the impact of results from symbolic analyses on the specifications generated by the LLM. The LLM prompts are augmented with outputs from two formal methods tools in the Frama-C ecosystem, Pathcrawler and EVA. We demonstrate how the addition of symbolic analysis to the workflow impacts the quality of annotations.

==> include/settings/Settings.tex <==
% CREATED BY DAVID FRISK, 2016

% CUSTOM
\usepackage{todonotes}

% BASIC SETTINGS
\usepackage{moreverb}								% List settings
\usepackage{textcomp}								% Fonts, symbols etc.
\usepackage{lmodern}								% Latin modern font
\usepackage{helvet}									% Enables font switching
\usepackage[T1]{fontenc}							% Output settings
\usepackage[english]{babel}							% Language settings
\usepackage[utf8]{inputenc}							% Input settings
\usepackage{amsmath}								% Mathematical expressions (American mathematical society)
\usepackage{amssymb}								% Mathematical symbols (American mathematical society)
\usepackage{graphicx}	
% Figures
\usepackage{subfig}									% Enables subfigures
\numberwithin{equation}{chapter}					% Numbering order for equations
\numberwithin{figure}{chapter}						% Numbering order for figures
\numberwithin{table}{chapter}						% Numbering order for tables
\usepackage{minted}						    		% Enables source code listings
\usepackage{chemfig}								% Chemical structures
\usepackage[top=3cm, bottom=3cm,
			inner=3cm, outer=3cm]{geometry}			% Page margin lengths			
\usepackage{eso-pic}								% Create cover page background
\newcommand{\backgroundpic}[3]{
	\put(#1,#2){
	\parbox[b][\paperheight]{\paperwidth}{
	\centering
	\includegraphics[width=\paperwidth,height=\paperheight,keepaspectratio]{#3}}}}
\usepackage{float} 									% Enables object position enforcement using [H]
\usepackage{parskip}								% Enables vertical spaces correctly 
\usepackage{datetime2} % date formatting tools - ISO-date YYYY-MM-DD
\usepackage{microtype} % Microtypography - improves readability and appearance of text.

\usepackage{mdframed}

% Allows clickable links for references, in table of content, autoref, etc.  	
\usepackage{hyperref}								
\hypersetup{colorlinks, citecolor=black,
   		 	filecolor=black, linkcolor=black,
    		urlcolor=black}

%% Bibliography https://www.overleaf.com/learn/latex/Bibliography_management_with_biblatex
\usepackage[style=ieee]{biblatex} % style=apa also possible
\addbibresource{references.bib}


% OPTIONAL SETTINGS (DELETE OR COMMENT TO SUPRESS)


		 

% Define the number of section levels to be included in the t.o.c. and numbered	(3 is default)	
\setcounter{tocdepth}{5}							
\setcounter{secnumdepth}{5}	


% Chapter title settings
\usepackage{titlesec}		
\titleformat{\chapter}[display]
  {\Huge\bfseries\filcenter}
  {{\fontsize{50pt}{1em}\vspace{-4.2ex}\selectfont \textnormal{\thechapter}}}{1ex}{}[]


% Header and footer settings (Select TWOSIDE or ONESIDE layout below)
\usepackage{fancyhdr}								
\pagestyle{fancy}  
\renewcommand{\chaptermark}[1]{\markboth{\thechapter.\space#1}{}} 


% Select one-sided (1) or two-sided (2) page numbering
\def\layout{2}	% Choose 1 for one-sided or 2 for two-sided layout
% Conditional expression based on the layout choice
\ifnum\layout=2	% Two-sided
    \fancyhf{}			 						
	\fancyhead[LE,RO]{\nouppercase{ \leftmark}}
	\fancyfoot[LE,RO]{\thepage}
	\fancypagestyle{plain}{			% Redefine the plain page style
	\fancyhf{}
	\renewcommand{\headrulewidth}{0pt} 		
	\fancyfoot[LE,RO]{\thepage}}	
\else			% One-sided  	
  	\fancyhf{}					
	\fancyhead[C]{\nouppercase{ \leftmark}}
	\fancyfoot[C]{\thepage}
\fi


% GEORGE'S ADDITIONS


\setlength{\marginparwidth}{2.5cm} 

\usepackage{listings}
\usepackage{xcolor}

\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}

\lstdefinestyle{cstyle}{
    language=C,
    basicstyle=\ttfamily\small,
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    breaklines=true,
    captionpos=b,                    
    keepspaces=true,                 
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2,
    moredelim=[is][\color{red}]{@@}{@@},
    }

\lstdefinestyle{csvstyle}{
    basicstyle=\ttfamily\footnotesize,
    columns=fullflexible,
    breaklines=true,
    postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
    frame=single,
    captionpos=b,
    showstringspaces=false,
    moredelim=[is][\textbf]{**}{**}
}

\lstdefinestyle{cotstyle}{
    basicstyle=\normalsize\ttfamily,
    language={},
    moredelim=[is][\color{red}]{@@}{@@},
}

\lstset{style=cstyle}

\usepackage{mdframed}
\newmdenv[
    linecolor=black,
    linewidth=2pt,
    backgroundcolor=gray!20,
    frametitlebackgroundcolor=gray!20,
    frametitlerule=true,
    roundcorner=10pt
]{mybox}

\usepackage{pgfplots}
\pgfplotsset{width=10cm,compat=1.16}



% Supress warning from Texmaker about headheight
\setlength{\headheight}{15pt}		

